Self-Sovereign Identity for Electric Vehicle Charging

Electric Vehicles (EVs) are more and more charged at public Charge Points (CPs) using Plug-and-Charge (PnC) protocols such as the ISO 15118 standard which eliminates user interaction for authentication and authorization. Currently, this requires a rather complex Public Key Infrastructure (PKI) and enables driver tracking via the included unique identifiers. In this paper, we propose an approach for using Self-Sovereign Identities (SSIs) as trusted credentials for EV charging authentication and authorization which overcomes the privacy problems and the issues of a complex centralized PKI. Our implementation shows the feasibility of our approach with ISO 15118. The security and privacy of the proposed approach is shown in a formal analysis using the Tamarin prover.

==> sections/adversary.tex <==

\section{Adversary Model}\label{sec:threat}

\todo{...}

==> sections/system_model.tex <==
\section{System Model}\label{sec:sysModel}

\todo{...}
